Towards 6G Holographic Localization: Enabling Technologies and Perspectives

In the last years, we have experienced the evolution of wireless localization from being a simple add-on feature for enabling specific applications to become an essential characteristic of wireless cellular networks, as for sixth-generation (6G) cellular networks. This paper illustrates the importance of radio localization and its role in all the cellular generations, from first-generation (1G) to 6G. Also, it speculates about the idea of holographic localization where the characteristics of electromagnetic (EM) waves, including the spherical wavefront in the near-field, are fully controlled and exploited to achieve better wireless localization. Along this line, we briefly overview possible technologies, such as large intelligent surfaces, and challenges to realize holographic localization. To corroborate our vision, we also include a numerical example that confirms the potentialities of holographic localization.

==> Definitions.tex <==

\newcommand{\Nb} {N_\mathsf{B}}
\newcommand{\Nm} {N_\mathsf{M}}
\newcommand{\Nl} {N_\mathsf{R}}
\newcommand{\Ns} {N}

\newcommand{\Hm} {\mathbf{H}}
\newcommand{\y} {\mathbf{y}}
\newcommand{\x} {\mathbf{x}}
\newcommand{\n} {\boldsymbol{\omega}}
\newcommand{\Hbm} {\mathbf{H}_\mathsf{BM}}
\newcommand{\Hbl} {\mathbf{H}_\mathsf{BR}}
\newcommand{\Hlm} {\mathbf{H}_\mathsf{RM}}
\newcommand{\bmOmega} {\bm{\Omega}}
\newcommand{\alphar} {\bm{\alpha}_\mathsf{r}}
\newcommand{\alphat} {\bm{\alpha}_\mathsf{t}}

\newcommand{\rhobm} {\rho_\mathsf{BM}}
\newcommand{\rhobl} {\rho_\mathsf{BR}}
\newcommand{\rholm} {\rho_\mathsf{RM}}
\newcommand{\rhoblm} {\rho_\mathsf{BRM}}

\newcommand{\tbm} {\tau_{bm}}
\newcommand{\tbl} {\tau_{br}}
\newcommand{\tlm} {\tau_{rm}}
\newcommand{\tdm} {\tau_{sm}}

\newcommand{\taubm} {\tau_\mathsf{BM}}
\newcommand{\taubl} {\tau_\mathsf{BR}}
\newcommand{\taulm} {\tau_\mathsf{RM}}
\newcommand{\taudm} {\tau_\mathsf{DM}}

\newcommand{\dbmo} {d_\mathsf{BM}}
\newcommand{\ddmo} {d_\mathsf{SM}}
\newcommand{\dblo} {d_\mathsf{BR}}
\newcommand{\dlmo} {d_\mathsf{RM}}
%\newcommand{\ddmo} {d_\mathsf{DM}}





\newcommand{\xilm} {\xi_{\mathsf{RM}}}
\newcommand{\etal} {\eta_r}
\newcommand{\etam} {\eta_m}

\newcommand{\xibm} {\xi_{\mathsf{BM}}}

\newcommand{\chibm}{\chi_{\mathsf{B}\mathsf{M}}}
\newcommand{\chiblm}{\chi_{\mathsf{B}\mathsf{R}\mathsf{M}}}

\newcommand{\phibm} {\phi_\mathsf{BM}}
\newcommand{\phibl} {\phi_\mathsf{BR}}
\newcommand{\philm} {\phi_\mathsf{RM}}
\newcommand{\phiL} {\phi_{\mathsf{R}}}
\newcommand{\phidm} {\phi_\mathsf{SM}}

\newcommand{\thetadm} {\theta_\mathsf{SM}}
\newcommand{\thetabm} {\theta_\mathsf{BM}}
\newcommand{\thetabl} {\theta_\mathsf{BR}}
\newcommand{\thetalm} {\theta_\mathsf{RM}}

\newcommand{\thetam} {\theta_m}
\newcommand{\thetab} {\theta_b}
\newcommand{\thetal} {\theta_l}

\newcommand{\xms} {x_{\mathsf{M}}}
\newcommand{\yms} {y_{\mathsf{M}}}
\newcommand{\zms} {z_{\mathsf{M}}}

\newcommand{\phim} {\phi_m}
\newcommand{\phib} {\phi_b}
\newcommand{\phil} {\phi_r}

\newcommand{\thetaL} {\theta_{\mathsf{R}}}

\newcommand{\dm} {d_{m}}
\newcommand{\dl} {d_{r}}
\newcommand{\db} {d_{b}}
\newcommand{\dbm} {d_{bm}}
\newcommand{\ddm} {d_{sm}}
\newcommand{\dbl} {d_{br}}
\newcommand{\dlm} {d_{rm}}
\newcommand{\fn} {f_n}

\newcommand{\xb}{x_b}
\newcommand{\yb}{y_b}
\newcommand{\nb}{w}
\newcommand{\zb}{z_b}

\newcommand{\xm}{x_m}
\newcommand{\ym}{y_m}
\newcommand{\zm}{z_m}

\newcommand{\xd}{x_s}
\newcommand{\yd}{y_s}
\newcommand{\zd}{z_s}

\newcommand{\Cbrm}{C_{brm}}
\newcommand{\BCr}{\bar{C}_{r}}
\newcommand{\BCk}{\bar{C}_{k}}
\newcommand{\Cbkm}{C_{bkm}}
\newcommand{\betam}{\beta_{m}}
\newcommand{\fc}{f_{0}}
\newcommand{\thetar}{\theta_r}
\newcommand{\thetak}{\theta_k}

\newcommand{\xdi}{x_d^{(0)}}
\newcommand{\ydi}{y_d^{(0)}}
\newcommand{\zdi}{z_d^{(0)}}

\newcommand{\xmi}{x_m^{(0)}}
\newcommand{\ymi}{y_m^{(0)}}
\newcommand{\zmi}{z_m^{(0)}}

\newcommand{\cosam}{c_{\alpha_{\mathsf{M}}}}
\newcommand{\sinam}{s_{\alpha_{\mathsf{M}}}}
\newcommand{\cosbm}{c_{\beta_{\mathsf{M}}}}
\newcommand{\sinbm}{s_{\beta_{\mathsf{M}}}}

\newcommand{\cosgm}{c_{\gamma_{\mathsf{M}}}}
\newcommand{\singm}{s_{\gamma_{\mathsf{M}}}}

\newcommand{\xl}{x_r}
\newcommand{\yl}{y_r}
\newcommand{\zl}{z_r}
\newcommand{\godm}{\mathsf{G}^{(1)}_{sm}}
\newcommand{\gobm}{\mathsf{G}^{(1)}_{bm}}
\newcommand{\gobl}{\mathsf{G}^{(1)}_{bl}}
\newcommand{\gtbm}{\mathsf{G}^{(2)}_{bm}}
\newcommand{\gtdm}{\mathsf{G}^{(2)}_{sm}}
\newcommand{\gtBM}{G_{\mathsf{B,M}}^{(b,m)}}
\newcommand{\gtDM}{G_{\mathsf{D,M}}^{(d,m)}}


\newcommand{\gtbl}{\mathsf{G}^{(2)}_{br}}
\newcommand{\gtlm}{\mathsf{G}^{(2)}_{rm}}
\newcommand{\gtLM}{G_{\mathsf{R,M}}^{(r,m)}}

\newcommand{\gtBL}{G_{\mathsf{B,R}}^{(b,r)}}
%\newcommand{\xb}{{x}_b}
%\newcommand{\yb}{{y}_b}
%\newcommand{\zb}{{z}_b}

%\newcommand{\xm}{x_{m0}}
%\newcommand{\ym}{y_{m0}}
%\newcommand{\zm}{z_{m0}}

%\newcommand{\xl}{x_{l0}}
%\newcommand{\yl}{y_{l0}}
%\newcommand{\zl}{z_{l0}}

\newcommand{\xmo}{x_{\mathsf{M}}}
\newcommand{\ymo}{y_{\mathsf{M}}} 
\newcommand{\zmo}{z_{\mathsf{M}}} 
\newcommand{\pmo}{\mathbf{p}_{\mathsf{M}}}

\newcommand{\pdo}{\mathbf{p}_{\mathsf{D}}}
\newcommand{\ado}{\boldsymbol{\Phi}_{\mathsf{D}}}
% \newcommand{\am}{\mathbf{a}_{\mathsf{M}}}
% \newcommand{\ab}{\mathbf{a}_{\mathsf{B}}}
% \newcommand{\al}{\mathbf{a}_{\mathsf{L}}}
\newcommand{\amo}{\boldsymbol{\phi}_{\mathsf{M}}}
\newcommand{\abo}{\boldsymbol{\Phi}_{\mathsf{B}}}
\newcommand{\alo}{\boldsymbol{\Phi}_{\mathsf{R}}}

\newcommand{\am}{{a}_{\mathsf{M}}}




\newcommand{\xbo}{x_{\mathsf{B}}}
\newcommand{\ybo}{y_{\mathsf{B}}} 
\newcommand{\zbo}{z_{\mathsf{B}}} 
\newcommand{\pbo}{\mathbf{p}_{\mathsf{B}}}

\newcommand{\xlo}{x_{\mathsf{R}}}
\newcommand{\ylo}{y_{\mathsf{R}}} 
\newcommand{\zlo}{z_{\mathsf{R}}} 
\newcommand{\plo}{\mathbf{p}_{\mathsf{R}}}

\newcommand{\hbm}{h_{bm}}
\newcommand{\hbl}{h_{br}}
\newcommand{\hlm}{h_{rm}}
\newcommand{\omegal}{\omega_{r}}

%\newcommand{\pbo}{\mathbf{p}_{\mathsf{B},0}}
\newcommand{\xbs}{{x}_{\mathsf{B}}}
\newcommand{\ybs}{{y}_{\mathsf{B}}}
\newcommand{\zbs}{{z}_{\mathsf{B}}}
\newcommand{\xds}{{x}_{\mathsf{D}}}
\newcommand{\yds}{{y}_{\mathsf{D}}}
\newcommand{\zds}{{z}_{\mathsf{D}}}
%\newcommand{\plo}{\mathbf{p}_{\mathsf{L},0}}
\newcommand{\xls}{{x}_{\mathsf{R}}}
\newcommand{\yls}{{y}_{\mathsf{R}}}
\newcommand{\zls}{{z}_{\mathsf{R}}}
\newcommand{\dant}{{d}_{\mathsf{ant}}}
\newcommand{\muBM} {\mu_{b,\mathsf{BM}}[n]}
\newcommand{\muBLM} {\mu_{b,\mathsf{BRM}}[n]}
\newcommand{\muBMc} {\mu^{*}_\mathsf{BM}[n]}
\newcommand{\muBLMc} {\mu^{*}_\mathsf{BRM}[n]}

\newcommand{\mubm} {\mu_{bm}[n]}
\newcommand{\cmubmp} {\mu_\mathsf{bm'}^*[n]}

\newcommand{\mublm} {\mu_{brm}[n]}
\newcommand{\mubmc} {\mu^{*}_\mathsf{bm}[n]}
\newcommand{\mublmc} {\mu^{*}_\mathsf{brm}[n]}



\newcommand{\alphamo}{\alpha_{\mathsf{M}}}
\newcommand{\betamo}{\beta_{\mathsf{M}}}
\newcommand{\gammamo}{\gamma_{\mathsf{M}}}

\newcommand{\Phim}{\Phi_{\mathsf M}}

\newcommand{\PEB}{\mathsf{PEB}}
\newcommand{\OEB}{\mathsf{OEB}}
